Compute-Efficient Deep Learning: Algorithmic Trends and Opportunities

Although deep learning has made great progress in recent years, the exploding economic and environmental costs of training neural networks are becoming unsustainable. To address this problem, there has been a great deal of research on *algorithmically-efficient deep learning*, which seeks to reduce training costs not at the hardware or implementation level, but through changes in the semantics of the training program. In this paper, we present a structured and comprehensive overview of the research in this field. First, we formalize the *algorithmic speedup* problem, then we use fundamental building blocks of algorithmically efficient training to develop a taxonomy. Our taxonomy highlights commonalities of seemingly disparate methods and reveals current research gaps. Next, we present evaluation best practices to enable comprehensive, fair, and reliable comparisons of speedup techniques. To further aid research and applications, we discuss common bottlenecks in the training pipeline (illustrated via experiments) and offer taxonomic mitigation strategies for them. Finally, we highlight some unsolved research challenges and present promising future directions.

==> figs_tables/mechanism_algorithm.tex <==
\begin{algorithm}[h]
\DontPrintSemicolon
 \caption{Algorithmically-Efficient Training}
 
  initial recipe $\leftarrow$ base configuration

 \tcc{Build speedup method}
 \tikzmk{A}
  element $\leftarrow$ one (or more) of the components

  action $\leftarrow$ one (or more) of the 5R speedup actions
 
 mechanism[how] $\leftarrow$ basis of action \tcp*[l]{Domain-knowledge or learning?}
 
 mechanism[when] $\leftarrow$ timing of action \tcp*[l]{Static or dynamic?}
 \tikzmk{B}
 \boxit{green}
 
 \tcc{Apply speedup methods with a static mechanism to baseline inputs} 
 \tikzmk{A}
 \KwIn{
 Function = \{architecture, model parameters\}
 
 \Indp \Indp \ Data = \{training dataset\}
 
 \ Optimization = \{training algorithm, training objective\}
 }
 
 \tikzmk{B}
 \boxit{blue}
 
 %initialize weights \;
 \tcc{Apply speedup methods with dynamic mechanisms to baseline training loop} 
 \tikzmk{A}
 \For(Optimization[algorithm])
 {$i := 1$ to $n_{\text{iteration}}$}
 {
    Data[samples] $\leftarrow$ batch from Data[dataset] \;
    Data[derived activations] $\leftarrow$ Function[architecture] applied to Data[samples] \;
    Data[derived gradient] $\leftarrow$ gradient of Optimization[objective] on Data[samples]\; 
    Function[model parameters] $\leftarrow$  updated based on Data[derived gradient] \;
 }\tikzmk{B}
 \boxit{pink}
 
\KwOut{Model trained to desired quality, \textit{faster}}
\end{algorithm}

